NFV-based IoT Security for Home Networks using MUD

A new scalable ISP level system architecture to secure and protect all IoT devices in a large number of homes is presented. The system is based on whitelisting, as in the Manufacturer Usage Description (MUD) framework, implemented as a VNF. Unlike common MUD suggestions that place the whitelist application at the home/enterprise network, our approach is to place the enforcement upstream at the provider network, combining an NFV (Network Function Virtualization) with router/switching filtering capabilities, e.g., ACLs. The VNF monitors many home networks simultaneously, and therefore, is a highly-scalable managed service solution that provides both the end customers and the ISP with excellent visibility and security of the IoT devices at the customer premises. The system includes a mechanism to distinguish between flows of different devices at the ISP level despite the fact that most home networks (and their IoT devices) are behind a NAT and all the flows from the same home come out with the same source IP address. Moreover, the NFV system needs to receive only the first packet of each connection at the VNF, and rules space is proportional to the number of unique types of IoT devices rather than the number of IoT devices. The monitoring part of the solution is off the critical path and can also uniquely protect from incoming DDoS attacks. To cope with internal traffic, that is not visible outside the customer premise and often consists of P2P communication, we suggest a hybrid approach, where we deploy a lightweight component at the CPE, whose sole purpose is to monitor P2P communication. As current MUD solution does not provide a secure solution to P2P communication, we also extend the MUD protocol to deal also with peer-to-peer communicating devices. A PoC with a large national level ISP proves that our technology works as expected.

==> background.tex <==
There are several ways in which IoT devices connect to the Internet:
Behind a broadband or cellular gateway, most commonly a customer premise equipment (CPE) router. The \iotica can be deployed at CPE broadband or cellular. It is important to note that the CPE  usually performs Network Address Translation (NAT) on outgoing connections.   

\ignore{
The device acts as another computer on the local network behind the gateway.  Sometimes the device resides behind multiple CPEs . The addresses of the IoT devices are within the protected network’s private address space, and are either fixed (static IP) or dynamic (using DHCP).  The CPE is directly connected to one or few CSPs and usually performs Network Address Translation (NAT) on outgoing connections.  The device itself is connected to the CPE either:
% * <dhay@cs.huji.ac.il> 2018-05-31T08:47:54.960Z:
% 
% יש כאן בלבול בין הדרך שבה אנחנו מתחברים ובין הפרוטוקול שבו אנחנו משתמשים:
% BT and the rest are protocols.
% so, (a) should be Ethernet IEEE 802.1
% (b) should be WLAN IEEE 802.11
% and then you have (c)
% 
% 
% ^.
\begin{enumerate}
\item Directly, by a physical e.g., 10BT cable.
\item Through a wifi connection.
\item Behind another IoT device or an IoT hub, to which a device may be connected by a low-energy short-range communication technology, such as Bluetooth, NFC, Zigbee, or Z-wave.
\end{enumerate}
\item Directly on a cellular network.
\end{enumerate}
}

%\begin{figure}[htb]
%\centering 
%\includegraphics[width=0.9\textwidth]{Background.png}
%\caption{\label{fig:Background.png} Direct connection and %cloud-based connection}
%\end{figure}

There are two common methods by which a user controls and monitors an IoT device via a smart mobile or a remote pc:


\begin{enumerate}

\item In {\em Cloud-based connection,} the IoT device acts as a client and opens a connection to one or more IoT specific services, that most usually are in the cloud.  To communicate with the IoT device, a user (through its smart device) connects to the IoT cloud service, which acts like a proxy between the user and the device.  In this model, the authorized endpoints of a device are the servers in the cloud, on which the IoT services reside.

\item In {\em Direct-based connection,} the user smart (mobile) device acts as a client opening a connection to the IoT device which acts as a server receiving commands from the user.  In this case, the user endpoint should know the network address (using DDNS or static IP address of the CPE) and the port number of the IoT device (configured on the CPE either by port forwarding and/or using uPnP).  Only authorized devices (owned by legitimate users) are allowed to initiate an incoming connection to the IoT device.  We note that direct-based connected devices can  still act as a client to other services used to maintain and update the IoT device itself (such as ntp).

\end{enumerate}


The cloud-based connection is more widely used and more secure due to the NAT service on the CPE and not having an open port to the wild Internet. Indeed the reported botnets, like MIRAI botnet \cite{MIRAI}, have used and broke into direct-connected IoT devices, by scanning the Internet and finding a device that had easy to crack password (including the CPEs themselves, that are a direct-based connected device). Notice that as reported in \cite{Shadon} there are still many IoT devices that are direct-connected and vulnerable in the Internet.  

The main threats on cloud-based connected devices are either that the cloud service has been compromised and it uploads a new firmware to the device, or the device is infected by another infected device on the same LAN.  The former is of low risk if the service is a secure cloud provider (which may not be always the case) while the latter is of somewhat higher risk.






















==> intro.tex <==
IoT devices are strong enough to host malicious code or become a zombie, but, for economical and technological reasons, they do not have the means to protect themselves from being hacked. Thus, the billions of IoT devices (estimates are from 10 to 50 billion by 2020, 50\% being consumer devices) are a fertile ground for many attacks of different kinds: DDoS attacks, privacy infringing attacks, data leakage, and physical break-ins. Several different systems and methods to provide protection to IoT devices have been proposed in recent years \cite{5,6,7,Meidan:2017:PML:3019612.3019878,IoTcities,DDoS_IoT}. In this paper we present an ISP level system that protects the IoT devices in a large number of homes. This effective scalable system should be a key part in protecting and stopping attacks on and from IoT devices.

The underlying property that distinguishes most IoT devices from home computers, such as laptops, desktops, and hand-held devices, is that in most cases an IoT device communicates with a limited number (most usually very small) of pre-defined domains. Furthermore, these devices, rarely if ever, go through a firmware update. These characteristics have been exploited to create a whitelist based protection methods for IoT devices. A recent widely used method, called Manufacturer Usage Description (MUD) \cite{jethanandani2018network,ietf-opsawg-mud-25}, requires the IoT device's vendor to provide the whitelist for its devices, called MUD file. Methods to automatically learn and acquire the MUD file for a device type have been also developed \cite{DBLP:journals/corr/abs-1804-04358}.

To protect an IoT device, given its MUD file, or any other whitelist, it is necessary to resolve the domain names in the list to get the corresponding IP addresses (which might be different in different geographies and at different times), then to monitor the device traffic ensuring it communicates only with the end points (IP addresses) it is authorized to communicate with, and if a deviation is detected, to deny or alert it by filtering any offending connection. Suggested implementations of the MUD standard as well as other IoT protection systems, implement these steps on premise internal/local area network, i.e., for home networks on the CPE, \cite{MCAFEE,ASUS,3,Heidmall,1,6,7,5,2,4}, though sometimes on a separate device. In this paper we provide a system architecture to implement these steps at the ISP level. The system combines a Virtual Network Function (VNF), holding the resolved MUD rules, that monitor a large number of homes (clients of the ISP) with enforcement capabilities on PoP (Point of Presence) routers or switches of the ISP, e.g., using ACLs. 

The IoT protection architecture suggested here has several advantages: First, it is not on the traffic critical path as in our PoC at a large local ISP, the VNF takes only a copy of the first packet of each connection. Secondly, the system correlates traffic surges and patterns from multiple homes to detect and mitigate outgoing DDoS attacks and other global attacks. Furthermore, being located upstream at the ISP the system is situated in a good point to stop incoming DDoS attacks on IoT devices and homes. Thirdly, we consider the CPE in each home as an IoT (regarding connections whose end point is in the CPE) and thus our system stops attempts to break into, and attacks that come out of, the CPE. Fourth, for any home whose CPE is managed by the ISP (the vast majority of homes) no cooperation from the client is necessary, the protection may be provided as a service in one click on the ISP management unit. Further notice, that the number of rules held in the VNF is proportional to the number of IoT device types (unique MUD files), and not to the total number of IoT devices it is monitoring.

Together with the above advantages, this system architecture possesses several challenges: First, the IoT devices reside behind a NAT which is part of the client CPE, thus making it difficult to identify the packets that come from specific devices, as all the traffic from a client premise comes with the same source IP address with arbitrary port numbers. Our design overcomes this difficulty using TR-69 to configure the client CPE (no need of client cooperation) to mark the devices' packets using different DSCP markings. A second challenge that is common to all whitelist approaches, are devices such as smartTVs, echo, etc., that may require a dynamic and larger whitelist, which should be updated on the fly. A third challenge introduced by our implementation is that the NFV unit at the ISP level does not monitor internal traffic in the client premise. Thus it does not detect attacks on IoT devices from other internal devices in same home. We therefore claim that a hybrid approach is necessary in order to enjoy all the benefits of the ISP based system and to stop internal attacks. Notice that the each part of the hybrid comlements the other and do different jobs. A final and non technical challenge is ISP incentives. Our approach requires investment from ISPs which they are not guaranteed to return by providing this protection as a manged service.

The focus of the current submission is implementing the MUD method at the ISP level. Below are other issues, some of which come with any MUD method implementation (or any other whitelist approach), which we deal with else where. First, some devices may be accessed directly by the owner mobile device(s) (peer2peer, P2P). In another work \cite{Hotnets} we propose methods to extend the MUD system to include the P2P connections in it, and these methods apply efficiently to our implementation. A second challenge, common to all whitelist based approaches, is posed by IoT vendors that place their services behind a cloud bucket (e.g., Amazon ec3 bucket), and on top use encrypted TLS communication with the bucket. An attacker mounting an attack from a (virtual) machine in the same bucket, will go undetected by the MUD whitelist. One approach to reduce this problem, is to use normal traffic patterns, at least for IoT services that run behind such buckets, and block or alert connections that exhibit abnormal behavior. 

More secure (at the ISP) since harder to tamper with and break the method.

QQQQQ

==> system.tex <==
\label{sec:system}
% -----------------------------
% A. Main components:  CPE, Guard, ISP Router, Agents. Cloud component 
% B. Guard operations: Acquiring Profiles (data plane part), Enforcing behavior % according to profile, what happened when a new device is joining home network 
%                                           Notice Profiles are not yet defined. 
% C. CPE Configuration (TR-69, ACS, etc.)
% D. Dealing with direct access iot devices
% E. Guard in the CPE or v-CPE
%
% -----------------------------------------------------
\label{sec:sys}This section describes in details the main components of \iotica framework, when the \iguard is deployed within the CSP network (namely, outside the customer premise), the IoT devices are cloud-based, and connected to the Internet through a CPE. In Section~\ref{sec:deployments}, there is a discussion on how our framework works for directly-connected IoT device, and how it should be adapted to settings where the \guard is deployed within the customer's network; namely, either as a standalone device in the network, a component within the CPE, or a component within a virtual CPE (v-CPE). We will also discuss further implementation details in Section~\ref{sec:implement}.

\iotica framework is built with a separate data-plane and control-plane, as illustrated in Figure~\ref{fig:framework}.

\begin{figure*}
\centering 
\begin{subfigure}{0.45\textwidth}
\includegraphics[clip, trim=0.5cm 3cm 0.5cm 3cm,width=\textwidth]{Dataplane.pdf}
\caption{\label{fig:dataplane} \iotica\negs's data-plane. }
\end{subfigure}
\quad\quad\quad\quad
\begin{subfigure}{0.45\textwidth}
\centering 
\includegraphics[clip, trim=0.5cm 3cm 0.5cm 3cm,width=\textwidth]{ContorlPlane.pdf}
\caption{\label{fig:controlplane} \iotica\negs's control-plane. }
\end{subfigure}
\caption{\label{fig:framework} The \iotica framework. In this example, \iguard protects two customers networks that communicate with the Internet through two CPEs. Both customer networks have camera installed in them, which connect to the same service in the cloud. \iguard contains profiles for all IoT devices in the system. In this particular case, it verifies that both cameras communicate only with endpoints within their profile}
\end{figure*}

\subsection{Data Plane}
\label{sec:dataplane}

\iotica\negs's data-plane, depicted in Figure~\ref{fig:dataplane}, deals with a single CSP network. It consists on three main parts: operations within the customers' private networks, operations within the CSP network, and the \iguard\negs, which monitors traffic and issues alerts (on abnormal behavior).



\subsubsection{Operations within the Customers' Network}

As mentioned before, we assume that customers connect to the CSP network through a \emph{Customer Premise Equipment} (CPE), which in most case is a gateway router. Typically, each CPE is allocated a unique IP address (which can change over time) within the CSP network address space. Each customer builds its own network, with a private address space, and may connect to it many devices (IoT devices or other devices). Each such device is allocated a private IP address and the CPE remaps its internal and external address spaces by performing \emph{Network Address Translation} (NAT). This implies that outside the customer network all packets use the same IP address (or addresses) and arbitrary ports (which are recorded at a dedicated NAT table within the CPE).  

IoT devices that are monitored by the \iotica framework are oblivious to its existence, and no special configuration need to be done at the IoT device level. 
However, as all packets that are transmitted from a single CPE use the same IP address, it is  difficult for routers, middleboxes, or network functions outside the customer premise to distinguish between traffic sent from different devices. Thus, CPEs that are connected to \iotica framework \emph{mark} packets originating from different IoT devices with different values of the DSCP field in the IP packet header. DSCP marking (by source MAC address) is a standard feature in most CPEs available today, and requires only CPE \emph{configuration}.\footnote{In the rare cases, where DSCP marking is not available, we use other methods such as accessing the NAT and ARP tables, manipulating NAT operations, using tunneling, and so on. We omit these methods for brevity.} We note that packets originating from non-IoT devices (such as desktops, laptops, or mobile phones) are not marked with a special DSCP value (and maintain the original value used by the device; $0$ in most cases). Newly-connected device, for which there is no indication whether it is an IoT device or not, is marked and tracked until such decision is made. The remote CPE configuration (namely, the assignment of a DSCP value for each device) is part of the control plane's operations as described in Section~\ref{sec:controlplane}.

We note that while packet marking may raise privacy concerns (as products can be identified behind the CPE's NAT), in our case, this is done with the customers' approval. Moreover, the same information can be obtained in other methods (e.g., by looking on unmarked DNS traffic~\cite{Apthorpe2016ASH,DENAT}) and is readily available in IPv6 deployments that do not use NAT at all.
%One may wonder, if marking packets originating from different IoT devices with different values (i.e., De-NAT) does not the harm the privacy rights of a customer. We do not think so, since even without marking one can categorize the IoTs in the customer network } using the DNS information. The marking is required only to ensure that a maleware cannot bypass the system, and mistakenly consider as traffic of other device in the system. Moreover, the alleged privacy is byproduct of the NAT, but not a feature of the network design. In fact in IPv6 in the common case there is no need of NAT, and every device will have its own IP address. 


\subsubsection{Operations within the CSP network}
After transmitted from the customer premise, packets are sent through a sequence of routers within the CSP network, towards their  destination. \iotica framework requires that one router along this route will \emph{copy} outgoing packets from all monitored customer premise and send them to the \iguard\negs. This can be done either using port mirroring or installing a specific filter on the CSP's router. Moreover, \iguard needs only \emph{one packet from each outgoing connection}\footnote{We define connection in this context as all packets that share the same $\langle src\_ip, src\_port, dst\_ip, dst\_port, protocol\rangle$ tuple.} as well as all DNS traffic from a customer premise. In case the router supports the OpenFlow protocols, for example, this can be done by dynamically installing a filter on every observed connection. 

We note that packets are \emph{copied} (and not routed) from the router to the ֿ\guard\negs, thus the \guard does not reside on the critical path of the packets, and does not induce extra delay or other performance penalties on the traffic.

The \guard may issue either alerts on abnormal behavior or access-control list (ACL) filters to block malicious traffic. In the latter case, these ACLs will be installed (either automatically or manually) either on the router that copied the traffic or on the respective CPE. \iguard has the capabilities to issue specific ACLs (e.g., block a specific connection; in most cases, both directions of the connection are blocked simultaneously) or aggregated ACLs (block all traffic to/from specific address/network; this is especially appealing in case of DDoS attack where many malicious connections are created simultaneously).

\subsubsection{Guard operations}
\label{sec:dp_guard}
The \iguard receives copies of the traffic of its customers. Packets have one of the following three DSCP values: (i) A commonly-used DSCP value, in which case we say that the packet is unmarked; (ii) A non-common DSCP value that the \guard uses as a default DSCP mark; (iii) Another non-common and non-default DSCP mark. The \guard handles the packets according to their packet marking:

\begin{description}
\item[{\bf Unmarked packets:}] \hspace{5.5em} Packets that have a DSCP value of $0$ (or another commonly-used value) were originated from a device that is not an IoT device, and therefore, is not monitored by \iguard\negs. Thus, \guard discards these packets.
\item[{\bf Marked packets of an identified IoT device:}] \hspace{17em} This consists of packets originating from a device that is known to be an IoT device, and its type is already known to the \guard\negs. This implies that one should only verify that the packets comply with the corresponding \emph{IoT profile}. Namely, in case the packet is a DNS query, the \guard extracts the queried domain name and verifies that it is in the profile's domain list. Otherwise, the \guard looks at the destination IP address of the packet, and verifies it corresponds to one of the domains in the profile (or to an hard-coded IP address). In case the \guard detects any deviation from the profile, it issues an alert. Such alert can indicate either that the IoT device was compromised or that the profile of the IoT device is no longer complete (e.g., due to a firmware update). See Section~\ref{sec:controlplane} on how alerts are handled and Section~\ref{sec:profile} on how profiles are being updated. 

\item[{\bf Marked packets of an unidentified device:}]  \hspace{16em} When a device joins a customer network, the CPE is configured to mark all its packet with a certain  value. In the beginning of the device operation, the \guard collects all of the device DNS queries and all the endpoints the device is communicating with. \guard compares (in an efficient manner) the list of domains and endpoints to all known profiles. If the device matches one of the profiles, the \guard associates these marked packets with the profile, and keeps tracking the device to ensure it continues to comply with the profile. Otherwise, the device is either an IoT device that has never been seen before (and therefore a new profile is created for it) or is not an IoT device (see Section~\ref{sec:profile}  for more details of how \guard distinguishes between these two cases). In the latter case, the \guard instructs the CPE to remove the DSCP mark from the device's packets, and therefore, all subsequent packets will arrive at the \guard unmarked.

We note that due to technical reasons there might be a gap between the time a device joins a customer's network and the time the corresponding CPE starts marking its packets. In order not to treat these first packets as unmarked, we configure the CPE to have a default proprietary DSCP value for all packets originating from the CPE. All such packets are treated as marked packets of an unidentified device, and the \guard associates them with the recently joined device (if only one such device exists).  See Section~\ref{sec:control_acs} for more details. 
%The \guard then configure the CPE, based on specific source MAC addresses,  either to mark packets or not to change the DSCP value of incoming packets (in case of non-IoT device).
\end{description}



%This poses a major challange on \iotica framework.


\subsection{Control Plane}
\label{sec:controlplane}

%TR-69
%Component in the cloud for directly-connected
%Alerts/visibility.


The control plane operations are divided into the following tasks that are executed periodically, when a new customer joins the framework, or when a new device joins an existing customer's network (namely, a new device is connected to the network for the first time). These operations are illustrated in Figure~\ref{fig:controlplane}.

\subsubsection{Maintaining data-plane's profiles}
\label{sec:activedns}
Notice that the \guard inspects marked non-DNS traffic only by looking at the destination IP address, and compares it with the addresses corresponding to the domains in the profile. Thus, the \guard needs to retrieve the IP addresses that are associated with the domains in the profile at the current location and time. 

One possibility is that the \guard could have retrieved these IP addresses by looking at the DNS responses to the DNS queries it already tracks. However, this implies that the \guard must see both directions of the traffic, which in some cases may not be available. Moreover, such a method does not protect against DNS poisoning attacks, as the DNS response might be bogus.

Alternatively, the \guard may perform \emph{active DNS queries} of the domains in all tracked profiles. This should be done periodically (e.g., every few minutes) to keep with changes of IP addresses.  Moreover, detection of a communication to an unidentified endpoint immediately triggers DNS queries of all domains in the profiles. This is done in order to verify that IP addresses did not change since the last active DNS query and thus eliminating false positives alerts.  In order to avoid learning malicious IP addresses due to DNS poisoning, the \guard may also store the common address space in the profile (per geographic location) or perform the DNS queries to a secure DNS server (such as OpenDNS or Quad9) that is immune to such attacks.

\subsubsection{Remotely Configuring CPEs}
\label{sec:control_acs}

One of the most important part of the control plane is the communication between the \guard to the CPE, in order to configure the latter. Such a configuration can be done in various ways, depending on the CPE capabilities. However, in the vast majority of cases, the CPE supports the TR-069 protocol for its remote configuration and CSP use this protocol to configure the CPE connected to their network. Thus, our description will focus on this protocol. Similar operations (and configurations) can be done using SNMP and proprietary management protocols. We note that once configuring a CPE, 
this configuration remains persistent (unless it is factory reset).  


TR-069~\cite{tr69} is a client-server protocol, where the CPE acts as a client and initiates connections to an \emph{Auto-Configuration Server} (ACS). This connections are initiated periodically (namely, once every \texttt{inform} interval). When a connection is established, the ACS sends configuration requests to the CPE, which are executed one by one. In addition, the ACS exposes a north-bound interface, so that management tools and applications can communicate with it. Thus, \iguard\negs, as any other TR-69--based application, communicates with the ACS (in our case, the CSP's ACS), which in turn, passes the requests to the CPE. An important feature of TR-069 is the ability to set a certain parameter for ``active notification''. In such a case, if the parameter  has been modified by an external cause (a cause other than the ACS
itself), the CPE initiates a connection immediately (without waiting to the next \texttt{inform} interval) to the ACS and notifies it on the parameter change. We will use this feature later to detect new devices that join the customer's network. 

The TR-069 supports data models that represent the entities that need to be configured. CPEs are modeled using the Internet Gateway Device (IGD) Data Model (TR-98)~\cite{tr98}, and the specific parameters our \guard uses are listed in Table~\ref{tab:tr98}; all the parameters are mandatory, implying that any CPE that supports TR-069 must support these configuration parameters. 

\input{tr69.tex}

Our \guard initiates configuration requests upon the following events:

\smallskip
\noindent
{\bf New customer is added to the network:} The external IP address of the customer is extracted (so that the \guard is able to identify connections from that customer). In addition, the respective TR-98 parameter in set to ``active notification'', so that future changes to the customer's external IP address will be reported automatically. Moreover, the \guard extracts basic details on all hosts that are connected to the CPE, and for each host it adds a mapping between its MAC address and a DSCP mark. 

In addition, it does the following operations: (i) adds a default DSCP mark (see Section~\ref{sec:dp_guard} for details); (ii) sets active notifications for the number of connected hosts (to detect hosts that join the customer's network); and (iii) extracts all port mappings configured on the CPE (for direct-based IoT devices, see Section~\ref{sec:DirectProfile})\footnote{Port mappings are also set to ``active notification'' to alert the \guard that a CPE opens or closed a new port.}. 

Finally, in many settings,  devices that are connected to the network are configured (through DHCP) to use the CPE as their DNS resolver. This implies that each DNS request is terminating in the CPE, which, in turn, issues another DNS request to CSP's DNS resolver, if needed. This implies that DNS requests arrive at the CPE unmarked. Since our data-plane tracks DNS queries, and since it is important to associate each query with the device that issued it, we change this configuration, so that each device communicates directly with the CSP's DNS resolver (and therefore, DNS requests arrive at the \guard with the correct DSCP mark). 
% We note marking DNS requests is important only when there are unidentified devices in the network. When all the devices are identified (which is the situation most of the time), we can revert to the default configuration. 

\smallskip
\noindent
{\bf External IP address is changed:} Recall that this parameter is marked for active notification, so that as soon as this happens, the CPE notifies the ACS (and then the \guard\negs) on this change. The \guard then updates its internal state to monitor connections/packets from the new external IP address rather than the old one.

\smallskip
\noindent
{\bf New device joins the network:} As the number of hosts connected to the CPE is marked for active notification, the ACS and the \guard are notified immediately upon such event. Then, basic details of the device (such as its MAC address, hostname, medium of connection, etc.) are extracted from the CPE, and the CPE is configured to mark all packets transmitted from this device. The \guard is configured to monitor these packets as well as to associate all packets with default mark to this device (to compensate on the time until the DSCP mark comes into effect). We note that, upon joining a network, all packets transmitted from the new device are marked packets of an unidentified device (see Section~\ref{sec:dataplane} for details on the \guard\negs's operations in such an event). 

We note that we consider a device as new only on the first time it connects to the CPE. If the device disconnects from the network and re-connects again, the CPE still lists it under its hosts (as inactive hosts), implying DSCP marks are already available, and no further action is required. 

\smallskip
\noindent
{\bf A device is classified as a non-IoT device by the \guard\negs:} In this case the DSCP mark on packets transmitted for this specific device should be removed, so that the \guard will stop monitoring the device by discarding the unmarked packets. This is done by setting the \texttt{DSCPMark} within the respective classification object to value -1, indicating that the CPE should not change the DSCP value of packets. Note that the classification object is not deleted, so that the device's packets will not be marked with the default DSCP mark we set earlier. 


\subsubsection{User Interface and Alerts}

The control plane of the \guard is also responsible to issue alerts to the users. Specifically, alerts are issued in one or more of the following events:
\begin{enumerate}
\item New device joins the customer's network.
\item An IoT device communicates with an unauthorized endpoint.
\item There is an activity on one of the CPE's open ports (for direct-based IoT devices, see Section~\ref{sec:DirectProfile}).
\end{enumerate}
Alerts are sent to the users either by a push notification (to a dedicated application), by email or as a text message. 

In addition, the control plane is the back-end engine of our user-interfaces, and therefore, is able to extract from the \guard all  data of a specific customer, all the alerts observed in the CSP network in a specific time-frame etc. (see Section~\ref{sec:implement} and Figure~\ref{fig:gui} \ignore{(in the appendix)} for further details on \iotica user interfaces). 

\subsubsection{Obtaining and disseminating profiles}

As we describe in details in Section~\ref{sec:profile}, based on the observed traffic, the \guard continuously finds new IoT devices, derives profiles for them, and keeps validating and updating the profiles it obtains (e.g., to capture firmware updates). 

As the \guard may be deployed in many CSPs, we keep an application outside the CSP network (namely, in the cloud), which receives the obtained profiles from the \guard\negs, and then disseminates new or updated profiles to all other \guard\negs s in the world. We note that as profiles typically contain domain names, each \guard will have to resolve the domain names by itself (see Section~\ref{sec:activedns}), which may results in different IP addresses due to differences in geographic locations of CSPs and/or resolving time. 

Moreover, we use \iotica\negs's cloud application to keep track on \emph{global phenomena}, such as large-scale cross-CSP DDoS attack or vulnerability in a specific device that has been observed in many CSPs simultaneously. 

\subsection{Dealing with directly-connected devices}
\label{sec:DirectProfile}

Unlike cloud-based IoT device, in a direct-based IoT devices, the communication is initiated by the end-user (e.g., her mobile device, desktop, or a server, which can be within or outside the CSP network), and is destined for the external IP address of the CPE. In the CPE, \emph{port forwarding} is configured so that all traffic that arrives at specific port $x$ is sent to a specific device $i$. Recall that these port mappings are obtained by the \guard when configuring the CPE (see Section~\ref{sec:controlplane}). 

As such devices do not have a \emph{profile} per se, in order to secure such devices, \iotica needs to obtain the legitimate endpoints for each device and/or the legitimate time in which such communication is possible.  

\iotica supports the following options:
\begin{description}
\item[{\bf Alert on every (new) activity:}]  \hspace{9em} In this option the \guard monitors all outgoing traffic from port $x$ and alerts the user on every connection to an IP address that was not seen before (or in recent time). In such a case, alerts will be sent for legitimate usage as well (so that the user can verify that the activity is indeed legitimate). If the user changes its IP address (e.g., when moving between networks), a new alert will be sent. Alerts can include also the type of protocol used for communication, as well as the volume of communication. 
\item[\bf{Whitelisting entire (sub-)networks:}]  \hspace{12em} In this option, the \guard is configured with a whitelist of sub-networks per customer. All direct communication for sub-networks on the whitelist to this specific CPE is allowed without alert, while \guard issues an alert for other communication. An example of a common whitelist is the address space of the cellular provider the customer is subscribed to, so that direct traffic from the customer's mobile phone is always allowed. Note that this option trades ease of operation with security, as it may allow attacker within any of the whitelist's sub-networks to directly access the customer's network.   
\item[{\bf Tracking the IP addresses of legitimate endpoints:}]  \hspace{19em} In this option, \iotica framework tracks the user's external devices and learns the IP addresses of them at any given time. For that, the user should install software (e.g., an application on the mobile device that can be a component within the CSP's mobile app), which has a unique identification mechanism that verifies that the user is indeed the one authorized to access the IoT device within the customer's network (e.g., using a digital signature or other off-the-shelf authentication mechanisms). Besides verifying the user credentials, the software also sends indication of the current IP address of each external device (such indication is sent either periodically or whenever an address is changed). \guard then uses the obtained IP addresses as whitelist, and alerts or blocks all other communication to port $x$. We note that for security reasons, the communication between these external devices and \iotica framework is done to \iotica's application in the cloud, which then sends securely the information the \guard component within the respective CSP network. 
\end{description}

As noted before, some IoT devices may use both direct- and cloud-based modes of operations. In such a case, cloud-based communication is monitored by the data-plane operations, as described in Section~\ref{sec:dataplane}, while direct-based communication (from the specific open port $x$) is monitored separately, as described above.

\subsection{Other Deployment Options for \iguard}
\label{sec:deployments}

While we described a specific deployment of \iotica framework, in which the \guard is deployed within the CSP network, there are  two other deployment possibilities.
\subsubsection{Deploying the \guard in the  customer's network} In this case, the \guard\negs's data-plane may be implemented in a stand-alone device or within the CPE, (either as part of the firmware or as an additional VM/Container that runs in the CPE). The \guard\negs's control-plane can be implemented in the same place, or might be implemented as a cloud service. In the latter case, the data-plane should communicate with that cloud service frequently, so that the cloud service will be able to collect information from different data-planes and disseminate information (such as profiles) back to the different data-planes. If the \guard is deployed within a CPE, we note that as the memory of the CPE is a scarce resource, the control-plane will disseminate only a subset of the profiles, to the IoT devices residing in its respective premise. This implies that device identification (see Section~\ref{sec:dp_guard}) is done entirely in the cloud. 

We note that when the \guard is deployed in the customer's network, it does have better visibility as it can observe and block unauthorized internal traffic between devices in the same network\footnote{This can be done to some extent by remotely configuring VLANs on the CPE.}. Moreover, packet marking is not required.  

On the other hand, deploying the \guard within the CPE suffers from memory (and processing) limitations of the CPE and may degrade its performance. Moreover, the solution is not generic and should be tailored to any new CPE type we encounter. Finally, \guard deployed in the CSP network should store a single copy of each profile for all the CSP customers, in contrast deployment in the CPEs this profile is copied again and again for each relevant subscriber. 

Stand-alone devices suffer almost from the same problems and tend to be the most expensive option to deploy. Moreover, the devices themselves should be managed, maintained, and monitored.

\subsubsection{\guard as a cloud service}

The \guard can be implemented in the cloud, where traffic is diverted or tunneled to a cloud-based service from the CPE (that, in turn, is configured to discard any traffic unless it comes from the cloud service).  In this scenario, both the data plane and the control plane are implemented as a cloud service.   The same cloud-based service, can handle traffic of multiple customers, and can be used, for example, to monitor multi-site enterprise networks. We note the cloud-based service in this scenario can reside either at some external cloud (e.g., as is done in another context by ZScaler~\cite{zscaler}), or within the CSP's private cloud. In the latter setting, this deployment is similar to deploying a v-CPE and having the \guard monitoring the traffic as one of the deployed network services.


\ignore{
the communication i
For direct connections between the user’s (mobile or desktop) device and the IoT device, the authorized endpoint is that user’s device. For the rest of the section, we refer to that device (whether it is a mobile phone, desktop, or any other media) as the external device. 
In such cases, endpoint identification is done by a user identification component installed on the external device. The profile then includes the pointer to the user (for example such as its phone number), from which the endpoint current IP address can be retrieved. 

The association between the software on the external device to the protected network may be done in a variety of ways. To name a few, one can verify that the installation is made while connected to the protected network (mostly applicable for mobile devices), using a dedicated password obtained from the ISP of the protected network, using off-the-shelf multi-factor authentication (MFA) mechanisms, and any combination of methods. The digital signature itself can be either a cryptographic signature, some cookie in the packet headers, data/meta-data that verifies the user with very high probability, or any other method that cannot be forged by a malicious agent.  I note that, as a security measure, my solution provides the users the details of all external devices that are authorized to access her protected network.

In normal operation, after the identification software has been placed on the user mobile device, the software sends to the enforcement apparatus, and specifically to its identification unit, information that includes the signatures that verify the user and the current IP address of the external device. These addresses become part of the profile for IoT devices in that user's premise. The information sent by the identification software can optionally also includes other information such as the usage of the IoT devices from that specific external device (e.g., the times at which the user opens an application/website that controls a specific IoT device). The information can give visibility of the usage of the IoT and verify traffic patterns. For example, one can correlate between the peak of traffic from a camera to the fact that the user's application has opened. Depending on the data-plane mode of operation this information, that includes the authorized endpoint IP, is sent either periodically, every time the external device changes its IPs address, or only before initiating a request to the IoT device.
If it is impossible to install such identification software on the external device, there are alternative ways to ensure that only legitimate users have initiated certain IoT activities.  For example, a notification to the user can be sent (for example, as an SMS) that notifies the user that a connection to the IoT device is attempted.  Then, like in two factor authentication, the user may approve or disapprove this attempt to connect with the IoT device (for example by sending back an appropriate SMS). 
}

% While in different architectures different components of the solution are placed in different network elements, there is one basic requirement that must always be satisfied:  it should be easy to identify connections from each specific IoT device.

%The two basic components of the solution are a data plane and a control plane.  These can reside in the same network element or in different network elements.   The data plane is the part that deals with the enforcement of the allowed and not allowed connections with different IoT devices. Namely, monitoring the traffic of IoT devices and filtering the traffic as necessary.  The control plane is the part that controls the data plane and configure it as necessary, including retrieving the authorized IP addresses of the endpoints, and managing the data plane. Below I mention several possible architectures. Some of them use the ability of already available network apparatus to perform part of the data path. 



\ignore{
4.1 Data plane

 

Monitoring and detecting deviations in the traffic (unauthorized accesses) may be performed in several different technologies depending on the architecture and network elements being used.  For example: one can use netflow, or Openflow, or any other SDN-based implementation, with or without port mirroring to the data-plane.  Alternatively, one can implement the data plane functionality directly in software.

Installing filters can be done using a variety of methods such as ACL on any of the routers in route from the IoT device to where the connection is going.  Alternative implementations could be Openflow rules in an SDN switch, TR69 to configure the filters on the subscriber router or by using any other networking device that uses filters to filter specific traffic. There are different actions that can be taken once a filter is matched. For example, beside filters with action of drop or allow, one can configure QoS, usually bandwidth, to different IoT devices.  This depends on the Guard’s mode of operation and detailed in Section 4.1.1. 

Marking packets of connections per IoT device is needed when some of the data-plane components are implemented outside the protected network. These components, which I call cloud components, usually cannot distinguish between packets originating from different devices within the same protected network, as the CPE (or other element in the protected network) performs Network Address Translation (NAT) before sending packets upstream. This implies that outside the protected network all packets use the same IP address (or addresses) and arbitrary ports (which is recorded at a dedicated NAT table).
To circumvent this problem, one option is to constantly retrieve the NAT table and send it to the cloud components.  The NAT table may be retrieved either by running software on the CPE or if a corresponding API to the retrieve the NAT table is available. With the NAT table, cloud components can associate an IoT device with certain ports and distinguish its traffic from the rest of the traffic.  
Another possible way is to mark all connections of a specific IoT device by a network element with such capabilities within the protected network (e.g., by the CPE). As the marking network element and the IoT device are on the same LAN, the marking network element can associate all packets originating from the IoT device by the source MAC address. In such a case, the control plane of the guard needs to configure the marking network element with the correct mark for each IoT device, and communicate this mark to the cloud components. One possible way of such marking is to configure the network marking element to set specific ToS bits on the packet according to the source MAC address, or by mapping different MAC addresses to different ports. In the common case where the network marking element is the CPE, the above configuration can be affected by the guard using control protocol such as TR069/TR098. Specifically, the control plane of the guard either runs or communicates with an Automatic Configuration Server (ACS) that sends the commands to the CPE over TR069 suite; alternatively, this can also be done using any other CPE control protocols (such as SNMP or proprietary APIs).  
Notice that when the protected network consists on a single IoT device (most commonly, an IoT device with a SIM card that connects directly to the cellular network), no packet marking is needed.
Special treatment to DNS queries of IoT devices: In the learning phase of a profile of a new IoT device, the algorithm needs to retrieve the DNS queries of a device.  However, in many cases the DNS queries from the IoT device are issued to a DNS resolver in the CPE. Then, the CPE issues a new query (in which the CPE is the source) to a resolver outside the protected network. This prevents a cloud component of the data plane to associate a query with the IoT device issuing it. One possible solution is that in the learning phase of a new device, the DNS resolver is configured to be a DNS outside the protected network (instead of the CPE). This is done using DHCP protocol in which DNS servers are typically configured. Moreover, in the typical case when DHCP server resides within the CPE, this configuration can be done using TR69 protocol. 


%4.1.1. Guard’s Mode of operations
%As explained before, filters are installed in the data-plane to detect communication with unauthorized endpoints. When such activity is detected by the filters, I offer several modes of operation, which can be configured either per an IoT device, a protected network, or an ISP:
%Detection Mode: In this mode, the filter is set to send log information on any traffic between the IoT device and the unauthorized endpoint. The log information is sent to alert the user (e.g., to his/her external device) or the ISP. The user or the ISP can then decide on further actions, which include switching to mitigation mode.
%The guard apparatus might process this log information and alerts on some global phenomena. For example, if an IoT device type causes alerts in many subscribers or protected networks at once, or if the same unauthorized endpoint appears in many of IoT devices type at once (this, for example, can be a strong indication of a botnet). 
%The processed information might also be shared with the IoT manufacture, which can be informed on a possible security breach in its products.  There is a trusted cloud interface in the control plane of the apparatus, in which vendor can respond to such breaches and verify the profiles of their products. 
%Mitigation mode: When un-authorized endpoint is identified a filter is set, in same network components along the route of the traffic (CPE, access router in the CPE or so on). 
%For direct-based connection, the default rule can be that no traffic to the IoT device is permitted and the rule that permits an endpoint to send traffic to the IoT device is installed just before the user indicates that she wants to activate the IoT device. The user can indicate her intentions either explicitly (e.g., using the software installed in her pre-authorized external device or SMS messages) nor implicitly (e.g., accessing a specific IoT device through its own application or website). Then, the guard apparatus can perform a check to verify the endpoints and if the endpoints is verified only then the filter is approved. This approach is less suited to cloud-based connection, since the IoT might constantly communicate with the authorized endpoints. Thus a rule per authorized endpoints might require too much rules, and is less scalable. 
%DDoS Mitigation Mode: In order to protect against DDoS attacks on the IoT device (namely, incoming DDoS attack), this mode permits all outgoing connections (namely, connection that where initiated from a device within the protected network; outgoing connections have packets on both directions) and all authorized endpoints to a directly-connected IoT device within the protected network. All other traffic is either blocked or rate limited in the ISP router. This ensures that all IoT devices (either directly connected or cloud-based) continue their normal operations, while malicious traffic is blocked away from the protected network. 



 }

==> tr69.tex <==
\begin{table}[th!]
\footnotesize
\begin{tabular}{|l|p{2cm}|}
\hline
\small{TR-98 Configuration Parameter} & \small{Meaning} \\
\hline\hline
\texttt{InternetGatewayDevice.WANDevice.\{i\}.} & External IP \\ 
\texttt{WANConnectionDevice.\{i\}.} &  address \\
WANPPPConnection.\texttt{\{i\}.ExternalIPAddress} & \\
\hline 
\texttt{InternetGatewayDevice.LANDevice.\{i\}.} & List of hosts   \\
\texttt{Hosts.host} & connected to a \\
&  CPE \\
\hline
\texttt{InternetGatewayDevice.QueueManagement} & An object that \\
\texttt{.Classification} & enables DSCP  \\
& marking by \hspace{-1em}\\
& source MAC address \\
\hline
\texttt{InternetGatewayDevice.WANDevice.\{i\}.} & List of open ports\\ 
\texttt{WANConnectionDevice.\{i\}.} &  on the CPE\\
WANPPPConnection.\texttt{\{i\}.PortMapping} & \\
\hline
\texttt{InternetGatewayDevice.LANDevice.\{i\}.} & DNS servers to  \hspace{-1em}\\
\texttt{LANHostConfigManagement.DNSServers} & be offered to   \\
& hosts during  \\
& DHCP\\
\hline

\end{tabular}
\caption{\label{tab:tr98} TR-98 Parameters we used to configure CPE connected to the \iotica framework. 
All parameters are mandatory since version 1.4 (September 2008).  }
\end{table}


